Adaptive Quadrilateral Mesh in Curved Domains

Nonlinear elliptic system for generating adaptive quadrilateral meshes in curved domains is presented. Presented technique has been implemented in the C++ language. The included software package can write the converged meshes in the GMV and Matlab formats. Since, grid adaptation is required for numerically capturing important characteristics of a process such as boundary layers. So, the presented technique and the software package can be a useful tool.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, ps, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a ps file, type "make ps".
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# Rouben Rostmaian
# September 2002

TEXFILE =  article.tex
#TEXFILE	= slides.texTPFA_diagonal_perm_variable.tex

.PHONY: dvi ps pdf clean

pdf:	$(TEXFILE:.tex=.pdf)
ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	( \
	\latex $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)

%.ps: %.dvi
	\dvips -q -t a4 $<

%.pdf: %.ps
	\ps2pdf -dPDFSETTINGS=/prepress $<

clean:
	@\rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.ps)

